Decision Theory-Guided Deep Reinforcement Learning for Fast Learning

This paper introduces a novel approach, Decision Theory-guided Deep Reinforcement Learning (DT-guided DRL), to address the inherent cold start problem in DRL. By integrating decision theory principles, DT-guided DRL enhances agents' initial performance and robustness in complex environments, enabling more efficient and reliable convergence during learning. Our investigation encompasses two primary problem contexts: the cart pole and maze navigation challenges. Experimental results demonstrate that the integration of decision theory not only facilitates effective initial guidance for DRL agents but also promotes a more structured and informed exploration strategy, particularly in environments characterized by large and intricate state spaces. The results of experiment demonstrate that DT-guided DRL can provide significantly higher rewards compared to regular DRL. Specifically, during the initial phase of training, the DT-guided DRL yields up to an 184% increase in accumulated reward. Moreover, even after reaching convergence, it maintains a superior performance, ending with up to 53% more reward than standard DRL in large maze problems. DT-guided DRL represents an advancement in mitigating a fundamental challenge of DRL by leveraging functions informed by human (designer) knowledge, setting a foundation for further research in this promising interdisciplinary domain.

==> Backup_for_long_related_work.tex <==
\item \zelin{(cold start problem, recommendation)} \cite{wei2017collaborative} presents a solution to the cold start (CS) problem in recommender systems by tightly integrating collaborative filtering (CF) and deep learning techniques. Leveraging the strength of the state-of-the-art CF model, timeSVD++, and a deep neural network SADE for content feature extraction, the study offers two novel models designed to address both complete cold start (CCS) and incomplete cold start (ICS) challenges. Comprehensive experiments on the large Netflix movie dataset demonstrated a significant enhancement in rating prediction accuracy for cold start items. Furthermore, the paper introduces a practical scheme for transitioning items from a cold start to non-cold start status, emphasizing a seamless user experience and effective promotion of cold start items in diverse online platforms. \\
\nithin{Motivation: The motivation behind this research lies in the need to accurately recommend Cold Start (CS) items to gather initial ratings, preventing them from receiving no ratings and improving overall recommendation system performance. Additionally, the study aims to estimate ratings for CS items, providing a measure of their potential popularity even before their market release, thus aiding in effective product planning and sales strategies. Accurate rating estimations are crucial for making informed decisions in this regard.}
\nithin{Goal: The primary goal of this research is to propose and evaluate recommendation models that can effectively handle cold start items, improving the prediction accuracy for such items. The authors specifically aim to develop separate models for CCS and ICS items. They combine time-aware collaborative filtering with deep learning architecture to extract item content features and account for temporal dynamics. By achieving this goal, the research seeks to advance the recommendation systems, particularly for challenging cold start scenarios. \\
Key Methodologies: The experiment involves a multi-step methodology to evaluate recommendation models for cold start items. Key steps include parameter configuration, preparation of training and test sets, model training using various algorithms, and rating prediction for performance assessment. These methods enable a comprehensive evaluation of the models' effectiveness in addressing the challenges of cold start items in recommendation systems. \\ Metrics:
The primary metric used to evaluate the performance of the proposed recommendation models is the Root Mean Square Error (RMSE). RMSE is a widely accepted objective metric for assessing the prediction accuracy of recommendation systems. It quantifies the disparity between predicted ratings and actual ratings, providing a measure of model performance. \\
Key Findings:
\begin{itemize}
\item The IRCD-CCS model, designed for CCS items, outperforms existing models for cold start items, achieving significant improvements in prediction accuracy compared to the ToA and ToU models.
\item  The IRCD-ICS model, tailored for ICS items, demonstrates superior accuracy compared to models such as ALS, SGD, timeSVD++, and CDL.
\item  The inclusion of time and item content information has a substantial impact on improving recommendation performance for both CCS and ICS items.
\item  The ICS item-based model is not effective for items with very few ratings, such as only 3 ratings. In such cases, it's recommended to use the CCS item-based model instead.
\end{itemize} \\
Limitations:
Firstly, the research primarily focuses on Netflix movie ratings data, potentially limiting the generalizability of its findings to other domains, indicating the need for caution when applying these findings to different contexts. Secondly, the aspect model's training and testing procedures might require further optimization to enhance its performance in rating imputation tasks. Lastly, the study evaluates performance using specific metrics, but it underscores the importance of recognizing that the choice of metrics and threshold values may vary according to the specific application and user preferences.}

\nithin{\item \jhc{out of scope} \cite{schein2002methods} This research paper investigates cold-start recommendations in recommender systems, focusing on predicting user preferences for items lacking prior ratings. It introduces the "Aspect Model," a probabilistic framework that combines content and collaboration information through EM learning. Comparative analysis with a naive Bayes method reveals varying system performance: the Aspect Model excels in implicit rating prediction, while the naive Bayes method outperforms in rating imputation. Heuristic recommenders are found to be effective in data-scarce scenarios. The study underscores the importance of appropriate evaluation metrics and acknowledges the complexity of cold-start recommendations, particularly for users with limited interaction data. Limitations include the focus on movie ratings data, the need for further optimization in the Aspect Model's procedures, and metric variability depending on specific applications and user preferences.}


\subsection{Are there any studies that also consider the use of game theory to solve the cold start problem in DRL?}
\begin{itemize}
    \item \cite{shaoyun2019coordinated} considered the game theory and DRL in research, but it's not focused on solving cold start.
    \item \cite{li2017deep} is a highly cited DRL survey paper. All existing DRL papers (until 2017) use game theory as a tool for creating games or for designing multi-agent DRL. No one has attempted to use game theory to solve the cold-start problem.
\end{itemize}

\nithin{\cite{ladosz2022exploration} This research paper explores the impact of initial entropy in deep reinforcement learning (DRL) on exploration and performance in discrete action space tasks. The goal is to address learning failures caused by low initial entropy and introduce an entropy-aware model initialization strategy to improve DRL algorithms. The study utilizes the Proximal Policy Optimization (PPO) algorithm and assesses DRL performance using reward metrics, discovering that low initial entropy increases the risk of learning failures. The proposed entropy-aware strategy mitigates this issue, leading to improved performance and faster learning in various tasks. However, limitations include its applicability to discrete tasks, the fixed entropy threshold choice, and a variable time overhead.}

\nithin{
Motivation:
The motivation behind this research is to explore the impact of initial entropy in deep reinforcement learning (DRL) on exploration and performance, specifically in tasks with discrete action spaces. The study aims to address the issue of learning failures caused by low initial entropy, which restricts exploration in early DRL training.\\
Goal:
The primary goal of this research is to analyze the effect of initial entropy on DRL performance, focusing on discrete action space tasks. Additionally, the study aims to introduce an entropy-aware model initialization strategy to mitigate learning failures, enhance performance, and accelerate learning speed in DRL algorithms. \\
Key Methodologies:
The study uses the Proximal Policy Optimization (PPO) algorithm to investigate the effect of initial entropy in discrete action space tasks. The entropy-aware model initialization strategy is introduced, which repeatedly initializes the model until the initial entropy surpasses a predefined threshold. This strategy aims to provide DRL algorithms with well-initialized models for improved exploration. \\
Metrics:
The research evaluates DRL performance based on rewards, learning failures, performance variations, and learning speed. It uses the average reward, standard deviation of rewards, and the minimum and maximum rewards as metrics to assess the effectiveness of the proposed entropy-aware model initialization strategy. \\
Key Findings:
1. Models with low initial entropy significantly increase the probability of learning failures, even in relatively simple tasks. \\
2. Initial entropy values tend to be biased towards low values, inhibiting exploration in DRL. \\
3. The proposed entropy-aware model initialization strategy reduces learning failures, enhances performance, decreases performance variations, and accelerates learning speed in DRL across various tasks and algorithms. \\
4. The time overhead of the proposed strategy is minimal relative to training times, and this overhead is primarily determined by action space size and initial entropy distribution, rather than task complexity. \\
Limitations:
- The study's findings are primarily relevant to tasks with discrete action spaces and may not directly apply to continuous control tasks. \\
- The choice of a fixed entropy threshold (0.5) may not be optimal for all tasks and scenarios. \\
- While the proposed strategy is effective, it introduces a time overhead that varies depending on the task and action space size, which could be a limitation in specific applications.} \\


\section{Related Work}
\subsection{Platforms for performance measuring}

The table \ref{tab:platforms} outlines key platforms utilized for assessing the efficacy of Deep Reinforcement Learning (DRL) algorithms and decision theory approaches. Notably, Gymnasium (formerly OpenAI Gym) is well known in DRL research for its extensive range of environments, from classic control tasks to Atari 2600 games. The Gym-Maze, specifically designed for the maze navigation problem, offers a unique challenge in testing the adaptability and efficiency of decision theory methodologies and DRL agents in complex, obstacle-laden environments.

\begin{table*}[h]
    \centering
    \begin{tabular}{l|l|l}
        \hline
        Platform & Description & Reference \\
        \hline
        Gymnasium (OpenAI Gym) & Varied environments for DRL & \cite{brockman2016openai}, \cite{towers_gymnasium_2023} \\
        Gym-Maze & 2D maze navigation & \cite{chan_gym-maze_2023} \\
        Atari 2600 (ALE) & Classic video game suite & \cite{bellemare2013arcade} \\
        MuJoCo & High-fidelity simulation & \cite{todorov2012mujoco} \\
        DeepMind Lab & 3D learning environments & \cite{beattie2016deepmind} \\
        \hline
    \end{tabular}
    \caption{Platforms for DRL and Decision Theory Evaluation}
    \label{tab:platforms}
\end{table*}

\subsubsection{Transfer Learning}

\cite{tessler2017deep} presents a Hierarchical Deep Reinforcement Learning Network (H-DRLN) approach to address the challenges of lifelong learning in the high-dimensional domain of the video game, Minecraft. The H-DRLN framework efficiently retains, reuses, and transfers knowledge across tasks by employing Deep Skill Networks (DSNs) as reusable skills. Two primary techniques, a deep skill array and a unique skill distillation method derived from policy distillation, enable the system to encapsulate multiple reusable skills into a single network, enhancing the efficiency and scalability of the learning process. Comparative analyses demonstrate the H-DRLN's superior performance and reduced sample complexity over the conventional Deep Q Network (DQN) when applied to Minecraft's sub-domains.

\mz{
 In \citet{genkin2022using}, a novel approach called Reinforcement Learning Building Optimizer with Transfer Learning (ReLBOT) is introduced. This technique is specifically developed to address the issue of smart building cold start. ReLBOT utilizes deep reinforcement learning and transfer learning to train an algorithm on a well-established smart building with a substantial historical data set. The trained algorithm is then applied to a new smart building that does not have any historical data available.
}

\subsubsection{Imitation learning}
\citet{gros2020tracking} introduces a novel approach to active imitation learning by reducing it to active i.i.d. (independent and identically distributed) learning, which allows leveraging advances in the i.i.d. setting to improve label efficiency in imitation learning. It presents the Reduction-based Active Imitation Learning (RAIL) algorithm and its practical variant, RAIL-DA, which incorporates data aggregation and incremental querying strategies. The technique is evaluated in various domains, including the Cart-pole environment, where RAIL-DA demonstrates significant effectiveness and efficiency by requiring fewer expert queries compared to passive learning approaches, thereby reducing the expert's labeling effort.

\citet{zou2020end} introduces the DDPG-IL algorithm, a framework combining Deep Deterministic Policy Gradient (DDPG) with imitation learning (IL) to enhance autonomous driving strategies. By initializing DDPG with IL-obtained strategies and employing a dual experience pool for optimal training data selection, DDPG-IL achieves faster convergence and superior performance compared to traditional DDPG. The effectiveness of this approach is validated through experiments in the TORCS racing simulator, demonstrating DDPG-IL's potential in efficiently learning driving strategies from expert data and self-improvement through continuous learning.

\subsubsection{Warm Start}


\cite{silva2021encoding} introduces Propositional Logic Nets (PROLONETS), a reinforcement learning (RL) technique that incorporates human domain expertise into the initialization phase of neural network training, aiming to "warm start" the learning process. By encoding domain-specific rules into the network via decision tree policies, PROLONETS bypasses the need for extensive datasets typically required for imitation learning (IL), thereby expediting the learning phase and reducing reliance on human labeling. The approach is empirically validated on OpenAI Gym tasks and modified StarCraft II tasks, demonstrating significant improvements in performance over traditional RL and IL methods. This system also shows an ability to engage with untrained humans. This validates its efficacy of incorporating human expertise into the RL framework. Nevertheless, this technique primarily focuses on enhancing decision trees or neural decision trees. How to integrate this method into established DRL algorithms like Q-learning and actor-critic has not been thoroughly investigated. Moreover, the transition from a guided model to a learner model within this technique is based on their entropy levels. Optimizing this transition could potentially be achieved by directly merging the knowledge from the guided model into the learner model.

\citet{wang2024flexnet} introduces FlexNet, a warm start method for deep reinforcement learning (DRL) in hybrid electric vehicle (HEV) energy management, enhancing the learning speed and energy efficiency. FlexNet encodes expert knowledge into a neural network's initial parameters, allowing for flexible architectural changes. This approach demonstrated significant improvements in learning speed (60.8\% and 88.8\% faster in different action spaces) and energy consumption (12.2\% and 6.4\% better than rule-based and equivalent consumption minimization strategies, respectively), showcasing its potential for efficient energy management in HEVs.

\mz{
The objective of \citet{xu2020learning} to decrease the number of learning iterations in Q-learning for hybrid electric vehicle (HEV) applications by employing warm-start methods. In contrast to previous studies that initialized Q-learning with zero or random Q values, this study commences Q-learning with various supervisory controls. The findings indicate that the proposed warm-start Q-learning necessitates 68.8$\%$ fewer iterations than cold-start Q-learning and enhances fuel efficiency by 10$\%$–16$\%$ when compared to the equivalent consumption minimization strategy control. These outcomes can be utilized to facilitate the implementation of reinforcement learning (RL) in vehicle applications.
}

\mz{
In \citet{wexler2022analyzing}, the degradation of Warm-Start RL (WSRL) is demonstrated by the authors through WSRL experiments in different environments. To address this degradation, they introduce a new approach called Confidence Constrained Learning (CCL) for WSRL. CCL reduces degradation by finding a balance between policy gradient and constrained learning, based on a confidence measure of the Q-values. The authors propose a novel objective, Positive Q-value Distance (CCLPQD), to design the constrained learning component. They explore several constraint-based methods to overcome the degradation and discover that these methods offer solutions for a multi-objective optimization problem, balancing maximal performance and minimal degradation.
}

\subsubsection{Sample Efficiency}
\cite{lin2021juewu} proposed a sample-efficient hierarchical Reinforcement Learning (RL) approach framework, called "JueWu-MC", specifically for open-world games like Minecraft. It addresses challenges such as partial observability, high-dimensional visual perception, and delayed rewards. Incorporating two hierarchical levels, it leverages human demonstrations, action-aware representation learning (A2RL), discriminator-based self-imitation learning (DSIL), and ensemble behavior cloning with consistency filtering. These innovations help the model to efficiently interpret and act within complex 3D environments, significantly outpacing contemporary baselines. Notably, this method clinched the top spot in the NeurIPS MineRL 2021 research competition, showcasing its effectiveness and promise in the domain of RL research.

\cite{den2022reinforcement} introduces a novel framework called Option Machines (OMs) for enhancing the sample efficiency of Reinforcement Learning (RL) by leveraging high-level, underspecified instructions. These instructions guide the selection and execution of temporally extended actions, known as options, within a hierarchical control structure. The key innovation lies in the use of Finite State Transducers (FSTs) to model the initiation and termination conditions for these options, allowing for complex behaviors like looping and interleaving of options based on environmental cues. The authors demonstrate that OMs can significantly outperform state-of-the-art methods in various settings, including single-task, multi-task, and zero-shot learning environments, even when instructions do not fully specify the tasks. This framework shows promise for real-world RL applications where complete task specifications are challenging to obtain, and the ability to reuse learned behaviors across tasks is crucial.


\mz{The authors in \citet{zhang2022coldstart} present a mathematical optimization problem to address the cold-start aware cloud-native Service Function Chains (SFC) caching problem. This problem incorporates a set of constraints that consider resource limitations and performance requirements.
A DRL method is proposed, named CSCA, which includes two embedding networks based on graph neural networks. These networks are used to extract information from the backbone network graph and caching requests. The DRL agent that is created is capable of learning caching decisions with the goal of optimizing the performance of processing latency, sub-frame processing latency, launch latency, and request acceptance ratio. Based on the simulation findings, CSCA demonstrates superior performance compared to other baseline algorithms in terms of the acceptance ratio of incoming requests, latency performance during high load, and handling of cold-start situations.}
